SemEval 2022 Task 12: Symlink- Linking Mathematical Symbols to their Descriptions

Given the increasing number of livestreaming videos, automatic speech recognition and post-processing for livestreaming video transcripts are crucial for efficient data management as well as knowledge mining. A key step in this process is punctuation restoration which restores fundamental text structures such as phrase and sentence boundaries from the video transcripts. This work presents a new human-annotated corpus, called BehancePR, for punctuation restoration in livestreaming video transcripts. Our experiments on BehancePR demonstrate the challenges of punctuation restoration for this domain. Furthermore, we show that popular natural language processing toolkits are incapable of detecting sentence boundary on non-punctuated transcripts of livestreaming videos, calling for more research effort to develop robust models for this area.

==> sec-data-analysis.tex <==
% \input{table-statistics}


==> sec-experiment.tex <==
\section{Experiments}

To assess the complexity of the Symbol Description Linking task in SciLink, we evaluate the performance of the state-of-the-art deep learning models for ED. In particular, the following models are tested:

\begin{itemize}

% REwrite and paraphrase to fit the task in this paper
    \item \textbf{OneIE} \cite{lin-etal-2020-joint}: OneIE is one of the state-of-the-art models in information extraction (IE) that is designed to jointly perform four tasks: entity mention detection, relation extraction, event detection, and argument role labeling. We adapt OneIE to our work using two tasks, i.e., entity mention detection and relation extraction. The model first detects the spans of entity mentions in the text. The detected spans are then paired to jointly predict entity types and relations. 
% REwrite and paraphrase to fit the task in this paper
    \item \textbf{FourIE} \cite{nguyen-etal-2021-cross}: FourIE is another state-of-the-art models for IE to simultaneously solves the four IE tasks in a single model. In addition, FourIE captures the inter-dependencies between prediction instances of different tasks by letting their representations interact with each other, hence, enhancing the predictions of the model. Similar to OneIE, we retain the two modules that perform entity mention detection and relation extraction, thus turning the model into a joint model for entity-relation extraction. This model is the best model on the ACE++ dataset \cite{Walker:05}.
    
    
% REwrite and paraphrase to fit the task in this paper
    \item \textbf{Jerex} \cite{eberts-ulges-2021-end} is a joint model for entity-level relation extraction from documents. Jerex introduces a multi-task approach that builds upon coreference resolution and gathers relevant signals via multi-instance learning with multi-level representations, combining global entity and local mention information. The model achieves state-of-the-art relation extraction results on the DocRED dataset \cite{yao-etal-2019-docred}.

\end{itemize}


\begin{table}[t]
    \centering
    \caption{Performance of the state-of-the-art models on SciLink dataset with references of performance on DocRED and ACE++ datasets. The numbers in the right most column show the performances of Jerex on DocRED dataset and OneIE and FourIE on ACE++ dataset. P, R, F stand for precision, recall, f1-score, respectively.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|ccc|ccc|c|}
        \hline
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Task}} & \mytitle{3}{Dev} & \mytitle{3}{Test} & \multirow{2}{*}{\textbf{F}}\\
        \cline{3-8}
        & & P & R & F & P & R & F & \\
        \hline
        \multirow{2}{*}{Jerex} & NER & \textbf{82.0} & 60.8 & 69.8 & \textbf{60.9} & 35.7 & 45.0 & 80.1\\
        & RE & \textbf{72.3} & 44.5 & 55.1 & 46.9 & 20.6 & 28.7 & 40.4\\ 
        \hline
        \multirow{2}{*}{OneIE} & NER &76.9 & \textbf{69.5} & \textbf{73.0} & 58.8 & 51.3 & \textbf{54.8} & 89.6\\
        & RE &61.4 & \textbf{54.2} & \textbf{57.5} & 34.2 & \textbf{31.1} & \textbf{32.6} & 58.6\\ 
        \hline
        \multirow{2}{*}{FourIE} & NER &75.3 & 68.4 & 71.7 & 55.1 & \textbf{52.2} & 53.6 & 91.1\\
        & RE &59.7 & 50.5 & 54.7 & 28.7 & 26.6 & 27.6 & 63.6\\
        \hline
    \end{tabular}
    }
    \label{tab:result}
\end{table}


\textbf{Hyper-parameters}: As the texts in this dataset are obtained from scientific documents, we use the \textit{allenai/scibert\_scivocab\_cased} version of SciBERT in all the considered models \cite{beltagy-etal-2019-scibert}. The Stanza toolkit \cite{qi-etal-2020-stanza}\footnote{https://stanfordnlp.github.io/stanza/} is employed for sentence splitting and dependency parsing. The hyper-parameters of the trained models are tuned over the development set based the suggested values from the original papers.

%Since the OneIE and FourIE models are designed for four tasks, we remove the modules that is designed for event detection, and argument role labeling tasks, while keep the named entity recognition and relation extraction modules.

\textbf{Results}: Table \ref{tab:result} reports the performance of the
models on the development and test sets of SciLink over two tasks: Entity Mention Detection (Entity) and Relation Extraction (Relation). Among the examined models, OneIE offers the best performance with F1 scores of 54.8\% for entity recognition and 32.6\% for relation extraction. For comparison, we also include the reported performances of these models on the DocRED and ACE++ datasets \cite{nguyen-etal-2021-cross,yao-etal-2019-docred}. As can be seen, the performance of the current information extraction models on SciLink is significantly and substantially worse than those on the DocRED and ACE++ datasets. For the entity recognition task, the F1-score difference between SciLInk and DocRED for Jerex is 35\%, and those between SciLInk and ACE++ for OneIE is 35\%. Due to the low performance of entity recognition, the relation extraction performance hurts sharply by up to 36\% between SciLink and ACE++ of the FourIE model. This suggests that the Symbol-Description Linking task in SciLink is a challenging task and more research effort is necessary to boost the performance of the models for this topic.

%and joint entity-relation extraction


==> table-example.tex <==
\newcommand{\hla}[1]{\colorbox{orange}{#1}}
\newcommand{\hlb}[1]{\colorbox{yellow}{#1}}
\newcommand{\hlc}[1]{\colorbox{cyan}{#1}}
\newcommand{\rota}[2]{\parbox[t]{3mm}{\multirow{#1}{*}{\rotatebox[origin=c]{90}{\textbf{#2}}}}}


\begin{table*}[t]
    \centering
    \caption{Tag schema for description recognition. The tag name and the entity mentions are highlighted accordingly.}
    \begin{tabular}{|l|l|p{12cm}|}
        \hline
        \rota{3}{Entity} & \hlc{Symbol} &  \hla{This set of class} is divided into \hlb{base and novel classes} \$\hlc{C\_b}\$ and \$\hlc{C\_n}\$, \\
        & \hla{Primary} &  respectively. Since customers care about fairness and infer subproportionally, \\
        & \hlb{Ordered} &\hla{the price elasticity of demand} is \$\hlc{E} = \textbackslash e+(\textbackslash e-1) \textbackslash g \textbackslash f(M\^p(P))\$ .\\
        \hline
        \rota{8}{Relations} & Direct &  The \hla{dataset} with data-label pairs \$\hlc{D} =\{(x\_i, y\_i)\}\$\\
        & & Finally, the monopoly has a constant \hla{marginal cost} \$\hlc{C}>0\$ \\
        \cline{2-3}
        &  &  The dataset with \hla{data-label pairs} \$D=\{(x\_i, y\_i)\} \textbackslash cdots \$ . \\
        & Coref-Description & \hla{The few available labeled data} are called support set \\
        && \$ \textbackslash mathcal\{S\}=\{(x\_i,y\_i)\}\$ \\
        \cline{2-3}
        & Coref-Symbol & It chooses price \$\hlc{P}\$ and output \$Y\$ to maximize profits \$(\hlc{P} - C) \textbackslash cdot Y\$ subject to customers' demand\\
        \cline{2-3}
        & Count &  $\cdots$ where every class in the task has $\hlc{q}$ \hla{test cases}. \\
        \hline
    \end{tabular}
    \label{tab:examples}
\end{table*}
